HyPar-Flow: Exploiting MPI and Keras for Scalable Hybrid-Parallel DNN Training using TensorFlow

To reduce training time of large-scale DNNs, scientists have started to explore parallelization strategies like data-parallelism, model-parallelism, and hybrid-parallelism. While data-parallelism has been extensively studied and developed, several problems exist in realizing model-parallelism and hybrid-parallelism efficiently. Four major problems we focus on are: 1) defining a notion of a distributed model across processes, 2) implementing forward/back-propagation across process boundaries that requires explicit communication, 3) obtaining parallel speedup on an inherently sequential task, and 4) achieving scalability without losing out on a model's accuracy. To address these problems, we create HyPar-Flow --- a model-size/-type agnostic, scalable, practical, and user-transparent system for hybrid-parallel training by exploiting MPI, Keras, and TensorFlow. HyPar-Flow provides a single API that can be used to perform data, model, and hybrid parallel training of any Keras model at scale. We create an internal distributed representation of the user-provided Keras model, utilize TF's Eager execution features for distributed forward/back-propagation across processes, exploit pipelining to improve performance and leverage efficient MPI primitives for scalable communication. Between model partitions, we use send and recv to exchange layer-data/partial-errors while allreduce is used to accumulate/average gradients across model replicas. Beyond the design and implementation of HyPar-Flow, we also provide comprehensive correctness and performance results on three state-of-the-art HPC systems including TACC Frontera (#5 on Top500.org). For ResNet-1001, an ultra-deep model, HyPar-Flow provides: 1) Up to 1.6x speedup over Horovod-based data-parallel training, 2) 110x speedup over single-node on 128 Stampede2 nodes, and 3) 481x speedup over single-node on 512 Frontera nodes.

==> text/backup.tex <==

System-oriented approaches to deal with out-of-core models have been investigated in ~\cite{awan-hipc18,dragon}.

However, data-parallelism has \underline{three fundamental limitations}: 1) Training the model to meet the accuracy of sequential training needs extensive hyperparameter (batch size, learning rate, etc.) search, which itself is a compute-intensive task, 2) Data-Parallel training has a synchronization (allreduce) overhead that can increase linearly with respect to the number of processes~\cite{gpipe,pipedream,lbann-ipdps19}, and 3) All DNN related data has to fit inside the device (CPU/GPU) memory. If the DNN does not fit inside device's memory, it cannot be trained and is referred to as an \textit{Out-of-core} model~\cite{vdnn,awan-hipc18,dragon}.






Significant challenges exist in exploiting \textit{model-parallelism} because the burden of partitioning the model is on the DNN designer, who is most likely a domain expert dealing with mathematical intuitions to design a model with better prediction capabilities for their use-case. Thus, there is a need for a user-transparent model-parallelism system that can automatically partition the model across multiple processes without any changes to the model definition as well as to the training process itself.

%Such an approach would also lead to very low productivity for the DNN designer since it will be manual effort for them to split the model and introduce explicit communication between model-partitions. Such a system will enable high-performance and high-productivity for DNN designers, which is currently not supported by existing frameworks.

%\MySubsection{Challenges}

\vspace{1.0ex}
\noindent \textbf{Challenges:} The key challenge we address in this paper is: \textit{How can we design a scalable and easy-to-use infrastructure for model, data, and hybrid-parallel training of DNNs that enables designers to 1) develop new type of DNNs without any restriction on its memory consumption and 2) train existing models with similar or better performance?} Along with the aforementioned broad challenge, we tackle the following concrete challenges in this paper:

\begin{itemize}
    \item What are the characteristics and features of a DNN that make them amenable to either model, data, or hybrid-parallelism? 
    
    \item Can model-parallelism be made as simple to use as the current set of data-parallelism approaches like Horovod~\cite{horovod}?
 
    \item How can we propose simple and unified APIs for parallel training that support multiple parallelization strategies (data, model, and hybrid)? 
    
    \item How can we effectively deal with communication across multiple processes that operate on different parts of a DNN in forward and backward passes?
    
    \item How to design efficient communication schemes when model and data parallelism is combined especially for complex models like ResNet(s)~\cite{resnet50} with non-consecutive layer connections?
    
\end{itemize}


------------


DESIGN

\MySection{HyPar-Flow: Proposed Architecture and Designs}
\label{sec:design}

We propose HyPar-Flow as an abstraction between the high-level ML/DL frameworks like TensorFlow and low-level communication runtimes like MPI as shown in Figure~\ref{fig:overview}. The HyPar-Flow middleware is directly usable by ML/DL applications and no changes are needed to the code or the DL framework. The four major internal components of HyPar-Flow, shown in Figure~\ref{fig:design-details}, are: 1) Model Generator, 2) Load Balancer, 3) Trainer, and 4) Communication Engine (CE).

\vspace{-5.0ex}
\mytwocolfigcustom  
{Overview of the Execution Stack}
{figures/hf-architecture.pdf}
{fig:overview}
{Major Components of HyPar-Flow}
{figures/hf-components.pdf}
{fig:design-details}
{HyPar-Flow: A Middleware for Hybrid-Parallel Training}
\vspace{-6.0ex}

\MySubsection{Designing Distributed Model Representation} 
\label{sec:modelgen}

The \textit{Model Generator} component is responsible for creating an internal representation of a DNN (e.g. a Keras model) suitable for distributed training (Figure~\ref{fig:teaser}). In the standard single-process (sequential) case, all trainable variables (or weights) of a model exist in the address space of a single process so calling \textit{tape.gradients()} on a \textit{tf.GradientTape} object to get gradients will suffice. However, this is not possible for model-parallel training as trainable variables (weights) are distributed among model-partitions. To deal with this, we first create a local model object on all processes using the \textit{tf.keras.model} API. Next, we identify the layers in the model object that are local to the process. Finally, we create dependency lists that allow us to maintain layer and rank dependencies for each of the local model's layers. These three components define our internal distributed representation of the model. This information is vital for realizing distributed back-propation (discussed next) as well as for other HyPar-Flow components like the \textit{Trainer} and the \textit{Communication Engine}. 

%for  dependenc. propose \textit{grad layers} (cf. Section~\ref{sec:trainer}).
%Because the model is distributed, we also create dependency lists for layers and save them in the Model Generator. The Trainer and the Communication Engine (CE) will utilize this information to realize model-parallel training on multiple model-partitions. 
%We designed the model generator such that it guarantees to follow sequential semantics for the distributed model-parallel version it creates. This is achieved by keeping all hyper-parameters including batch size, learning rate, and training steps exactly the same as in sequential training. This is to make sure that there is no effect whatsoever on the accuracy of the training process. We note that this guarantee does not apply to data-parallel training as it averages the gradients across model-replicas so it is only semantically similar to serial training, \textit{in expectation}~\cite{maleki-msr-ipdps18}.

\MySubsection{Implementing Distributed Back-Propagation}
\label{sec:trainer}

Having a distributed model representation is crucial. However it is only the first step. The biggest challenge for HyPar-Flow and its likes are: ``How to train a model that is distributed across process boundaries?''. We deal with this challenge inside the \textit{Trainer} component. First, we analyze how training is performed on a standard (non-distributed) Keras model. Broadly, there are two ways to do so: 1) \textit{model.fit(..)} and 2) \textit{model.train\_on\_batch(..)}. Second, we explore how we can design an API that is very similar to the standard case. To this end, we expose a single \textit{hf.fit(..)} interface that take parallelization strategy as an argument. The value of the \textit{strategy} argument can be model, data, or hybrid. Third, we design a custom training loop for distributed back-propagation for the model/hybrid parallel case. For data-parallel, it is not needed because the model is replicated on all processes instead of being distributed across processes.


%\textit{data-parallel} training, we simply use something called a \textit{DistributedGradientTape} from the Horovod library to get the gradients and then call \textit{apply\_gradients()} on the \textit{tf.optimizer} object. 
%The symbols used are summarized in Table~\ref{tab:symbols}. 

We show a very simple DNN in Figure~\ref{fig:simplenet} to explain back-propagation and highlight what needs to be done for realizing a distributed version. In addition to Figure~\ref{fig:simplenet}, we use Equations 1--7 to provide a more detailed explanation. There are three key data elements in DNN Training: 1) The input $X$, 2) The predicted output $Y'$, and 3) The actual output (or label) $Y$. The intermediate output from the hidden layer is denoted as $V$. The difference between $Y$ and $Y'$ is called error or loss labeled as $L$ (Eq.~\ref{eq:1}).

\begin{figure}[htbp]
    \centering
    \vspace{-5.0ex}
    \includegraphics[width=0.6\columnwidth]{figures/nn.pdf}
    \vspace{-2.0ex}
    \caption{A Neural Network with a single Hidden layer}
    \vspace{-2.0ex}
    \label{fig:simplenet}
\end{figure}



\input{text/equations.tex}

To realize distributed back-propagation, we need: 1) partial derivative (D1) of Loss $L$ with respect to the weight $W1$, and 2) partial derivative (D2) of Loss $L$ with respect to the weight $W2$. The challenge for multi-process case is that the term called ``partial error'' shown in Equations~\ref{eq:6} and~\ref{eq:6} can only be calculated on \textit{Partition-2} (Figure~\ref{fig:simplenet}) as $Y'$ only exists there. To calculate D1, \textit{Partition-1} needs this ``partial error'' term in addition to D1. Because we rely on accessing gradients using the DL framework's implementation, this scenario poses a fundamental problem. TensorFlow, the candidate framework for this work, does not provide a way to calculate gradients that are not part of a layer. To implement this functionality, we introduce the notion of \textit{grad layer} in HyPar-Flow, which act as pseudo-layers inserted before the actual layer on each model-partition. We note that TensorFlow's \textit{GradientTape} cannot be directly used for this case. \textit{Grad layers} ensure that we can call \textit{tape.gradients()} on this \textit{grad layer} to calculate the partial errors during back-propagation. Specifically, a \textit{grad layer} is required for each \textit{recv} operation so that partial error can be calculated for each preceding model-partition's input. A call to tape.gradients() will return a list that contains gradients as well partial errors. The list is then used to update the model by calling \textit{optimizer.apply\_gradients()}.
%\lstinputlisting[language=Python, caption={Realizing Model-Parallel Training in HyPar-Flow using \textit{tf.GradientTape} and \textit{optimizer.apply\_gradients()}},label={code:comm}]
%{"code/comm.py"}
%Listing~\ref{code:comm} shows the pseudo-code for HyPar-Flow's implementation of this distributed model-parallel back-propagation.

We note that there is no need to implement distributed back-propagation for data-parallel case as each model-replica is independently performing the Forward and Backward pass. The gradients are only synchronized (averaged) at the end of the Backward pass (back-propagation) using \textit{allreduce} to update the model weights in a single step. 

%We also investigate \textit{the use of tape.gradients() to calculate partial errors} that are needed to realize model-parallel back-propagation for TensorFlow.


%\textit{tf.keras.model} and {tf.GradientTape} to  API Basic Design of Distributed Model a Model-Definiti}

\MySubsection{Realizing Inter-Partition and Inter-Replica Communication}
\label{sec:ce}

In Sections~\ref{sec:modelgen} and~\ref{sec:trainer}, we discussed how distributed model definition is generated and how back-propagation can be implemented for a model that is distributed across processes. However, \textit{Trainer} and \textit{Model Generator} only provide an infrastructure for distributed training. The actual communication of various types of data is realized in HyPar-Flow's \textit{Communication Engine (CE)}. The CE is a light-weight abstraction for internal usage and it provides four simple APIs: 1) send, 2) recv, 3) broadcast, and 4) allreduce. 

\vspace{1.0ex}
\noindent \textbf{HyPar-Flow CE Basic Design:} For pure data-parallelism, we only need to use allreduce. However, for model-parallelism, we also need to use point-to-point communication between model-partitions. In the forward pass, the send/recv combination is used to propagate \textit{activations} from each partition to the next partition starting at \textit{Layer 1}. On the other hand, send/recv is used to back-propagate the \textit{loss} and \textit{partial-errors} from one partition to the other starting at \textit{Layer N}. Finally, for hybrid-parallelism, we need to introduce allreduce to accumulated (average) gradients across model replicas. We note that this is different from the usage of allreduce in pure data-parallelism because in this case, the model itself is distributed across different partitions so allreduce cannot be called directly on all processes. One option is to perform another p2p communication between model-replicas for gradient exchange. The other option is to exploit the concept of MPI communicators. We choose the latter one because of its simplicity as well as the fact the MPI vendors have spent considerable efforts to optimize the allreduce collective for a long time. To realize this, we consider the same model-partition for all model-replicas to form the \textit{Allreduce communicator}. Because we only need to accumulate the gradients local to a partition across all replicas, allreduce is called on this communicator will suffice. Please refer back to Figure~\ref{fig:teaser} in Section~\ref{sec:intro} for a graphical illustration of this overall scheme. 


\vspace{0.5ex}
\noindent \textbf{HyPar-Flow CE Advanced Design:} The basic CE design described above works but does not offer good performance. To push the envelope of performance further, we investigate two HPC optimizations: 1) we explore if overlap of computation and communication can be exploited for all three parallelization strategies and 2) we investigate if pipelining can help overcome some of the limitations that arise due to the sequential nature of forward and backward passes. Finally, we also handle some advanced cases for models with non-consecutive layer connections (e.g. ResNet(s)), which can possibly lead to deadlocks. 

\vspace{0.5ex}
\noindent \textit{Exploiting Overlap of Computation and Communication:} In order to achieve near-linear speedups for data-parallelism, overlap of computation (forward/backward) and communication (allreduce) has proven to be an excellent choice. Horovod, a popular data-parallelism middleware, provides this support so we do simply use it inside HyPar-Flow for pure data-parallelism. However, for hybrid-parallelism, we design a different scheme. We create one MPI communicator per model partition whereas the size of each communicator will be equal to the number of model-replicas. This design allows us to overlap the allreduce operation with the computation of other partitions on the same node. An example scenario clarifies this further: if we split the model across 48 partitions, then we will use 48 allreduce operations (one for each model-partition) to get optimal performance. This design allows us to overlap the allreduce operation with the computation of other partitions on the same node. 

\vspace{0.5ex}
\noindent \textit{Exploiting Pipeline Stages within Mini-batches}

Model and data-parallelism can be combined in a myriad of ways to realize hybrid-parallel training. E.g. model-parallelism on a single node with multiple cores with data-parallelism across nodes. There are non-trivial and model-dependent trade-offs involved when designing hybrid schemes, which are beyond the scope of this paper.  

We need multiple MPI communicators to efficiently overlap computation and communication when Allreduce (for data-parallelism) is combined with Send/Recv (for model-parallelism).

Model-Parallelism and data-parallelism have different use cases. We have seen that model-parallelism is beneficial when we have a large model, or we want to keep a small batch size for training. On the other hand, Data-Parallelism gives a near-linear scale-up performance as we increase the number of nodes, but it also increases batch size. We also observe that on a single node model-parallelism gives better performance compared to data-parallelism by utilizing multiple model-partitions on a single node, but the number of model-partitions can not be larger than the number of layers in the model. Therefore we cannot increase the number of model-partitions beyond a certain point in model-parallelism. For example, we can not have more than 101 partitions for ResNet-101 model, but in practice, one layer per model-partition did not give the best performance. Therefore, we have included hybrid-parallelism in HyPar-Flow so that it can benefit from both model and data-parallelism. Performance on Hybrid-Parallelism depends on how well the combination of model-parallelism and data-parallelism performs and also how it is implemented under the hood.



Figure~\ref{fig:deadlock-avoidance} shows a non-consecutive model with skip connections that requires communication 1) between adjacent model-partitions for boundary layers and 2) non-adjacent model-partitions for the skip connections. To handle communication dependencies among layers for each model-partition, we create two lists: 1) Forward list and 2) Backward list. Each list is actually a list of lists to store dependencies between layers as shown in Figure~\ref{fig:deadlock-avoidance}. ``F'' corresponds to index of the layer to which current layer is sending its data and ``B'' corresponds to index of the layer from which the current layer is receiving data. An arbitrary sequence of sending and receiving messages may lead to a deadlock. For instance, if \textit{Partition-1} sends the partial predictions to \textit{Partition-3} when \textit{Partition-3} is waiting for predictions from \textit{Partition-2}, a deadlock will occur as \textit{Partition-2} is itself blocked (waiting for) results from \textit{Partition-1}. To deal with this, we sort the message sequence according to the ranks so that the partition sends the first message to the partition which has the next layer. 

\begin{figure}[htbp]
\centering
    \includegraphics[width=0.6\textwidth]{figures/deadlock-new.pdf}
    \caption{Realizing Communication in HyPar-Flow. The direction of arrows shown in the figure is to illustrate communication in the Forward Pass only. The communication will happen in the reverse direction for the Backward Pass.}
    \label{fig:deadlock-avoidance}
\end{figure}


%Inside the HF class, we instantiate the \textit{Model Generator} to create a hybrid-parallel version of the model. We then utilize the \textit{Trainer} and \textit{Communication Engine} to train the model across multiple processes in an efficient manner. For expert users, we also allow an additional input we call \textit{LPP}. LPP stands for Layers Per Partition, and is a simple array of the form $[n1, n2, ..., nk]$ where $k$ is the number of total partitions (for MP) and $nk$ is the number of layers for partition $k$. This additional input is optional and is only for experts who already understand their system and model characteristics. It can also be a good knob for designers who want to experiment and benchmark their models as well as the HyPar-Flow system. The use of \textit{LPP} is shown in Listing~\ref{code:HyPar-Flow}.



